FRuDA: Framework for Distributed Adversarial Domain Adaptation

Breakthroughs in unsupervised domain adaptation (uDA) can help in adapting models from a label-rich source domain to unlabeled target domains. Despite these advancements, there is a lack of research on how uDA algorithms, particularly those based on adversarial learning, can work in distributed settings. In real-world applications, target domains are often distributed across thousands of devices, and existing adversarial uDA algorithms -- which are centralized in nature -- cannot be applied in these settings. To solve this important problem, we introduce FRuDA: an end-to-end framework for distributed adversarial uDA. Through a careful analysis of the uDA literature, we identify the design goals for a distributed uDA system and propose two novel algorithms to increase adaptation accuracy and training efficiency of adversarial uDA in distributed settings. Our evaluation of FRuDA with five image and speech datasets show that it can boost target domain accuracy by up to 50% and improve the training efficiency of adversarial uDA by at least 11 times.

==> chapters/extras.tex <==
\subsection{Computing Wasserstein distance across distributed datasets} 
\label{subsec.dist_wass}
Our optimal collaborator selection algorithm requires computing an estimate of the Wasserstein ($W_1$) distance between a candidate domain ($D_C$) and the target domain ($D_T$). Let  $X_{C}$ and  $X_{T}$ denote the unlabeled datasets from the two domains. As shown by \cite{shen2018wasserstein}, the $W_1$ distance can be computed as:  
\begin{align}
\text{$W_1$} (X_{C}, X_{T}) = \frac{1}{n_{C}} \sum_{x_{s} \sim \mathcal X_{C}} DI(E_{C}(x_{c})) - \frac{1}{n_{T}} \sum_{x_{t} \sim \mathcal X_{T}} DI(E_{T}(x_{t}))
\label{eq:wass_impl}
\end{align}
where $n_{C}$ and $n_{T}$ are the number of samples in the dataset, $E_{C}$ and $E_{T}$ are the feature encoders of each domain, and $DI$ is an optimal discriminator trained to distinguish the features from the two domains. To train the optimal discriminator, following loss is minimized: 
\begin{equation*}
\min\limits_{DI} \mathcal L_{adv_{DI}} = -{\mathbb{E}}_{x_{c} \sim \mathcal X_{C}, x_{t} \sim \mathcal X_{T}} [W_1 (x_{c}, x_{t}) + \gamma L_{grad}]
\end{equation*}
where $L_{grad}$ is the gradient penalty used to enforce 1-Lipschitz continuity on the discriminator. 

Interestingly, Equation~\ref{eq:wass_impl} has a similar structure to the optimization objectives for ADDA and other uDA algorithms discussed in the paper. Hence, we can use the same principle as DILS and exchange discriminator gradients between nodes to compute the Wasserstein Distance in a distributed manner, without requiring any exchange of raw data. 

We initialize $E_T$ with $E_C$ and decompose the discriminator $DI$ into two parts ($DI_C$ and $DI_T$) which reside on the respective nodes. The raw data from both nodes is fed into their respective encoders and discriminators, and we compute the gradients of each discriminator as follows:

\begin{equation*}
\mathcal L_{DI}^{^C}  = \frac{1}{n_{C}} \sum_{x_{s} \sim \mathcal X_{C}} DI_C(E_{C}(x_{c})) 
\end{equation*}
\begin{equation*}
\mathcal L_{DI}^{^T} = \frac{1}{n_{T}} \sum_{x_{t} \sim \mathcal X_{T}} DI_T(E_{T}(x_{t}))
\end{equation*}


\begin{minipage}{.5\linewidth}
\begin{equation*}
\nabla g(DI_C, x_c) = \frac{\delta \mathcal L_{DI}^{^C}}{\delta DI_C}
\end{equation*}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\begin{equation*}
\nabla g(DI_T, x_t) = \frac{\delta \mathcal L_{DI}^{^T}}{\delta DI_T}
\end{equation*}
\end{minipage}

Both nodes exchange their discriminator gradients during a synchronization step and compute aggregated gradients:  

\begin{equation}
\nabla g(DI_\mathrm{agg}, x_c, x_t) = \nabla g(DI_C, x_c) - \nabla g(DI_T, x_t)
\end{equation}

Finally, both discriminators $DI_C$ and $DI_T$ are updated with these aggregated gradients, and gradient penalty is applied to enforce the 1-Lipschitz continuity on the discriminators. This process continues until convergence and results in an optimal discriminator. Once the discriminators are trained to convergence, we can calculate the Wasserstein distance as:


% The gradient penalty is applied to enforce the 1-Lipschitz continuity on both discriminators. As shown in \cite{gulrajani2017improved}, gradient penalty is computed on data points sampling uniformly along straight lines between pairs of points in $X_{C}$ and $X_{T}$. In other words, 


% computed as $\gamma x_c + (1 - \gamma) x_t$ 



\begin{equation*}
\text{$W_1$} (X_{C}, X_{T}) = \mathcal L_{DI}^{^C}  - \mathcal L_{DI}^{^T}
\end{equation*}


\subsection{Privacy Analysis of DILS} 
\label{subsec:dils.privacy}
Recall that a key feature of our distributed training algorithm is to exchange information between the distributed nodes using \emph{gradients of the discriminators}. This clearly affords certain privacy benefits over existing uDA algorithms since we no longer have to transmit raw training data between nodes. However, prior works have shown that model gradients can potentially leak raw training data in collaborative learning \cite{melis2019exploiting}, therefore it is critical to examine: \emph{can the discriminator gradients also indirectly leak training data of a domain}? 

We study the performance of DILS under a state-of-the-art gradient leakage attack proposed by \cite{zhu2019deep}. They showed that gradient matching can be a simple but robust technique to reconstruct the raw training data from stolen gradients. Let us say we are given a machine learning model $F()$ with weights $W$. Let $\nabla W$ be the gradients with respect to a private input pair $(\mathbf{x},y)$. During distributed training, $\nabla W$ are exchanged between the nodes. 

A reconstruction attack happens as follows: an attacker first randomly initializes a dummy input $\mathbf{x'}$ and label input $y'$. This data is fed into the model $F()$ to compute dummy gradients as follows:

$$
\nabla W^{\prime}=\frac{\partial \ell\left(F\left(\mathbf{x}^{\prime}, W\right), \mathbf{y}^{\prime}\right)}{\partial W}
$$

Finally, the attacker minimizes the distance between the dummy gradients and the actual gradients using gradient descent to reconstruct the private data as follows:

\begin{equation}
\begin{aligned}
\mathbf{x}^{\prime *}, \mathbf{y}^{\prime *}&=\underset{\mathbf{x}^{\prime}, \mathbf{y}^{\prime}}{\arg \min }\left\|\nabla W^{\prime}-\nabla W\right\|^{2} \\
&=\underset{\mathbf{x}^{\prime}, \mathbf{y}^{\prime}}{\arg \min }\left\|\frac{\partial \ell\left(F\left(\mathbf{x}^{\prime}, W\right), \mathbf{y}^{\prime}\right)}{\partial W}-\nabla W\right\|^{2}
\label{eq:attack}
\end{aligned}
\end{equation}

\textbf{Can this attack succeed on DILS?} There are two key assumptions in this attack: (i) the weights $W$ of the end-to-end machine learning model are available to an adversary in order for them to compute the dummy gradients, (ii) the gradients of all the layers ($\nabla W$) between the input $x$ and output $y$ are available to the adversary.  

DILS never exchanges the weights of the target domain model (i.e., the feature extractor and the discriminator) during the adversarial training process. As shown in Algorithm 1, the target feature extractor is trained locally and only discriminator gradients are exchanged. Without the knowledge of the model weights $W$, an attacker can not generate the dummy gradients $\nabla W'$ necessary to initiate the attack on the target domain. 

Looking at the source or collaborator domain, we do exchange its feature extractor with the target domain in the initialization step of uDA, which could be used by the attacker to generate the dummy gradients $\nabla W'$. However, for the attack to succeed, the attacker also needs the real gradients ($\nabla W$) of all the layers between the input $x$ and output $y$ in the source domain. This includes gradients of $E_S$ and $DI_S$. In DILS however, we only exchange the gradients of the domain discriminator $DI_S$ during training; the gradients of $E_S$ are never exchanged. Without the knowledge of the gradients of $E_S$, an attacker cannot use Eq.~\ref{eq:attack} to reconstruct the training data of the source domain. 

In summary, we have proven that our strategy of distributed uDA based on discriminator gradients does not allow an attacker to reconstruct the private data of either the source or the target domain. 
